Still Not Quite There! Evaluating Large Language Models for Comorbid Mental Health Diagnosis

In this study, we introduce ANGST, a novel, first-of-its kind benchmark for depression-anxiety comorbidity classification from social media posts. Unlike contemporary datasets that often oversimplify the intricate interplay between different mental health disorders by treating them as isolated conditions, ANGST enables multi-label classification, allowing each post to be simultaneously identified as indicating depression and/or anxiety. Comprising 2876 meticulously annotated posts by expert psychologists and an additional 7667 silver-labeled posts, ANGST posits a more representative sample of online mental health discourse. Moreover, we benchmark ANGST using various state-of-the-art language models, ranging from Mental-BERT to GPT-4. Our results provide significant insights into the capabilities and limitations of these models in complex diagnostic scenarios. While GPT-4 generally outperforms other models, none achieve an F1 score exceeding 72% in multi-class comorbid classification, underscoring the ongoing challenges in applying language models to mental health diagnostics.

==> sections/table_IAA.tex <==
\begin{table}[!t]
\begin{center}
\small % Reducing the font size
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\begin{tabular}{lcc}
\toprule
 & \textbf{Anxiety} & \textbf{Depression} \\
\midrule
\textbf{Krippendorff's alpha ($\alpha$)} & $0.423$ & $0.622$ \\
\textbf{Fleiss' kappa ($\kappa$)} & $0.444$ & $0.624$ \\
\bottomrule
\end{tabular}
\end{center}
\caption{Inter-annotator between annotators for anxiety and depression labels. We report Krippendorff's alpha and Fleiss' kappa scores respectively for each label.}
\label{tab:IAA_agreement}
\end{table}
